Untrimmed Video Classification for Activity Detection: submission to ActivityNet Challenge

Current state-of-the-art human activity recognition is focused on the classification of temporally trimmed videos in which only one action occurs per frame. We propose a simple, yet effective, method for the temporal detection of activities in temporally untrimmed videos with the help of untrimmed classification. Firstly, our model predicts the top k labels for each untrimmed video by analysing global video-level features. Secondly, frame-level binary classification is combined with dynamic programming to generate the temporally trimmed activity proposals. Finally, each proposal is assigned a label based on the global label, and scored with the score of the temporal activity proposal and the global score. Ultimately, we show that untrimmed video classification models can be used as stepping stone for temporal detection.

==> text/soa.tex <==
\section{Related work}

%----------------action classification---------------------
Many approaches to action recognition \cite{laptev-2008,wang-2011,wang-2013} are based on appearance (e.g., HOG \cite{dalal-2005} or SIFT \cite{Lowe-2004}) or motion features (e.g., optical flow, MBH \cite{dalal-2006}),
encoded using Bag of Visual Words or Fisher vectors.
The resulting descriptors are typically used to train classifiers (e.g. SVM) in order to predict the labels of action videos.
%-----------------cnn based action classification and localisation--------------------
Recently, however, inspired by the record-breaking performance of CNNs in image classification \cite{krizhevsky2012} and object detection from images \cite{girshick-2014}, deep learning architectures have been increasingly applied to action classification \cite{Shuiwang-2013,Karpathy-2014,Simonyan-2014} and localisation \cite{Georgia-2015a,Weinzaepfel-2015}.

For instance in global action classification,
Simonyan and Zisserman \cite{Simonyan-2014} have proposed a novel feature extraction approach based on two Convolutional Neural Networks (CNNs),
one encoding static appearance features from RGB images, and the other extracting motion features from optical flow heat maps.
Gkioxari and Malik \cite{Georgia-2015a} have extended the work of \cite{girshick-2014} and \cite{Simonyan-2014} to tackle both classification and localisation.
Moreover, Weinzaepfel at al. \cite{Weinzaepfel-2015} use a tracking-by-detection approach based on a novel track-level descriptor (Spatio-Temporal Motion Histogram, STMH) combined with CNN features.
%They use a sliding-window approach to temporally segment an action.
The downside of the aforementioned approaches is that they perform localisation of actions in videos which only contain one action.
Furthermore, the action videos are already temporally trimmed and therefore it is hard to evaluate their temporal localisation.

%-------------------------cnn based contextual action recog and localisation ----------
In order to improve action recognition and localisation, Georgia  \etal\  \cite{Georgia-2015b}  and and Jain  \etal\  \cite{Jain-2015},
use CNN features and add contextual cues.
Whereas the work of Georgia \etal\ is limited to localisation in still images,
the approach by Jian \etal\ will only reap benefits where the objects in the action are discriminative.
In some of the actions in the LIRIS-HARL dataset, categories such as `unsuccessfully unlocking door' and `successfully unlocking door' both have the same set of objects. In this case, the object `door' does not reveal any additional information about the action.

%\cmt{Suman what are you tryin gto say here?}
%Lan  \etal\  \cite{Lan-2011} learn spatio-temporal models for actions using figure-centric visual word representation, where the location of the subject is treated as a latent variable and is inferred jointly with the action label.
%--------------------action localisation-------------
% recog and localisation
%Tian  \etal\  \cite{tian-2013} attempted to detect and localise actions from videos by extending the deformable parts model \cite{felzenszwalb-2010} tailored for object recognition in 2D images, to video using HOG3D feature descriptors \cite{klaser-2010}.

% have made advance in temporal localisation but they do not address the problem of sptial localisation and co-ocurring actions, as only one action occur at time in whole frame. 
%  Afore mentioned methods do try t address the problem of temproal action detection but lack in spatail localisations.  
%All the aforemention state-of-the-art approaches are focused on action classification or localisation,
%in which each video clip contains a single action and has been manually trimmed in time.

The temporal localisation actions~\cite{jiang2014thumos,gorban2015thumos}, events~\cite{TRECVID} and gestures~\cite{escalera2014chalearn} in temporally untrimmed videos has attracted much attention recently.
These challenges led to big advances in the state-of-the-art \cite{yeung2015every,xu2014discriminative}.
%Xu  \etal\  \cite{xu2014discriminative} propose to encode teh last convolutional layer of CNN into VLAD and Fisher vector representations.
However, unlike our work, these approaches address only the temporal action localisation.
For multiple co-occurring actions in time, Yeung \etal\ introduced a Long Short Term Memory network \cite{yeung2015every}.
They augmented the annotation on the Thumos Dataset \cite{jiang2014thumos} to include new categories and co-occurring actions;
the downside is that spatial localisation information has been ignored.

Multiple concurrent action detection from temporally untrimmed videos has only been explored on a small number of action classes.
For instance Laptev \etal\ proposed an action detection approach based on \textit{keyframe priming}~\cite{laptev-2007}.
Their idea was to improve space-time interest point detectors for actions such as `drinking',
with single frame detection from state-of-the-art methods in object detection.
Alternatively, \cite{klaser-2010} split action detection into two parts: i) detecting and tracking humans,
and ii) using a space-time descriptor and sliding window classifier to detect the location of two actions (phoning and standing up).
By contrast we consider 10 different action categories.

In this paper we propose a novel action detection method which addresses the challenges involved in classification, localisation and detection of co-occurring actions in space-and-time given temporally untrimmed videos. 

%- THE SOA IS A BIT UNSTRUCTURED, WHY NOT KEEP THE DIVISION IN PARAGRAPHS USED FOR GOOGLE PROPOSAL?
%- FINALLY, MAYBE A TABLE COMPARING OUR FEATURES TO THOSE OF MAIN COMPETITORS COULD BE GOOD TO PUT

